Finding Multiple New Optimal Locations in a Road Network

We study the problem of optimal location querying for location based services in road networks, which aims to find locations for new servers or facilities. The existing optimal solutions on this problem consider only the cases with one new server. When two or more new servers are to be set up, the problem with minmax cost criteria, MinMax, becomes NP-hard. In this work we identify some useful properties about the potential locations for the new servers, from which we derive a novel algorithm for MinMax, and show that it is efficient when the number of new servers is small. When the number of new servers is large, we propose an efficient 3-approximate algorithm. We verify with experiments on real road networks that our solutions are effective and attains significantly better result quality compared to the existing greedy algorithms.

==> planar.tex <==
\section{Almost Planar Networks}

Road networks are almost planar: compared to the total number
of road segments, the number of bridges and tunnels is very small.
Therefore, techniques developed for planar graphs will often also work for
road networks. Here we consider another way to decompose the graph by means of
the Planar Separator Theorem [56], which states that for any planar graph
with n nodes, there is a node set of size $O(\sqrt{|V|})$, a so-called separator,
whose deletion leaves two components consisting of at most $2/3 |V|$  nodes
each.


%Only deal with the boundary points.

%There are about $0.03|V|$ boundary points.

%Assume clients, servers, all lie on boundary points.

\subsection{Separator}

A graph is said to be embedded in a surface S when it is drawn on S so that no two edges intersect.
A graph is planar if it can be embedded in the plane.
%A plane graph has already been embedded in the plane.
We refer to the regions defined by a plane graph as the faces.
The unbounded region is called the exterior face.

Let $G$ be an embedded planar graph.
Let T be a BFS spanning tree for $G$ and $L(i)$ be the
set of nodes at level $i$ in $T$.
Clearly $L(i)$ is a separator since
T is a BFS tree.
Let $F(e)$ denote the fundamental cycle determined by T and some non-tree edge.
$F(e)$ is a separator since T is a spanning
tree for $G$.
Lipton and Tarjan's separator theorem is based on 
combining the two
kinds of separators in order to
obtain a separator of size $O(\sqrt{n})$.

Let $l_1$ be the level in T such that
$\sum_{i=0}^{l_1-1} |L(i)| < n/2$ but
$\sum_{i=0}^{l_1} |L(i)| \geq n/2$.

Search up T at most $\sqrt{n}$ levels from $l_1$ to
locate a level $l_0 \leq l_1$ (which must exist) such that
$|L(l_0)| \leq \sqrt{n}$.
Similarly, search down T from $l_1$ at most $\sqrt{n}$ levels to locate a level $l_2 \geq l_1$ such that $L(l_2)| \leq \sqrt{n}$. ``Cut'' T at the levels $l_0$ and $l_2$, dividing it
into three ``pieces'' $G_1$, $G_2$, and $G_3$ (see Fig. 1).
Cutting the nodes at a level involves the removal of all nodes on that level, together with all of their incident edges, of which there can be at most $O(n)$, since $G$'s being planar implies that $|E|$ is $O(n)$. If the middle piece, $G_2$, is of size at most $2n/3$, then we are done. So suppose that $|G_2| > 2n/3$. Create a new root $r$ and join $r$ to all the roots of subtrees created when we cut T at $l_0$. This creates a spanning tree $T_2$ of $G_2$ that has depth at most $2 \sqrt{n}$. Lipton and Tarjan show that there is a fundamental cycle $F(e)$ in $G_2$ (whose size must be $O(\sqrt{n})$ that separates $G_2$ into two graphs of size at most $2n/3$. Adding this cycle to the nodes in $L(l_0)$ and $L(I_2)$ gives us an $O(\sqrt(n))$-separator for $G$, and all this can be easily in $O(n)$ time.

Question: 
The separated components may be disconnected and the connected parts can be far away from each other on the plane. However, we would like to preserve connectivity and compactness of the components.
if we stop at connected components satisfying the size criteria, instead of targeting at the separated components in the original design (which may be disconnected), can we maintain the guarantee of the size of separator vertices ?

%\subsection{Definitions}
%
%A graph is said to be embedded in a surface S when it is drawn on S so that no two edges intersect.
%A graph is planar if it can be embedded in the plane.
%A plane graph has already been embedded in the plane.
%We refer to the regions defined by a plane graph as the faces.
%The unbounded region is called the exterior face.
%
%A cutpoint of a graph is one whose removal increases the number of components, and a bridge is such a line.
%
%A nonseparable graph is connected, nontrivial, and has no cutpoint.
%
%A block of a graph is a maximal nonseparable subgraph.

%\subsection{Line Graphs}
%
%Let $G$ be a graph, Sedlacek has shown that the line graph of $G$ is planar iff $G$ is planar, the degree of each vertex in $G$ is at most 4, and every vertex of degree 4 is a cutpoint.

\subsection{Plane sweep}

To derive the intervals $I$ in a road network R such that
$I$ maximizes the total weight of the line segments that fully cover $I$, we can apply a standard plane sweep algorithm on the line segments in $R$.  

\subsection{Bridges and Tunnels}

A road network is not totally planar, since there can be bridges and tunnels. 

==> ref.tex <==
R. J. Lipton and R. E. Tarjan. A separator theorem for planar graphs.
SIAM Journal on Applied Mathematics, 36(2):177–189, April 1979.
